Measuring Information Leakage in Website Fingerprinting Attacks and Defenses

Tor provides low-latency anonymous and uncensored network access against a local or network adversary. Due to the design choice to minimize traffic overhead (and increase the pool of potential users) Tor allows some information about the client's connections to leak. Attacks using (features extracted from) this information to infer the website a user visits are called Website Fingerprinting (WF) attacks. We develop a methodology and tools to measure the amount of leaked information about a website. We apply this tool to a comprehensive set of features extracted from a large set of websites and WF defense mechanisms, allowing us to make more fine-grained observations about WF attacks and defenses.

==> allfeatures.tex <==
\section{All Features}

% talk with Nick about Feature set. I just notice that the reviewer's comments was updsated once. So what I knew is not accurate. 
% the reviewer argues about the feature set. Yes, I agree with him that our results depend heavily on what features are selected. I should be careful in selecting features. Nick's advice is to refer it to the importance of using entropy to measure the system. I will write about the basic ideas behind it. 


% I am wondering whether combining features can do good or not. I am curious about the chemistry in combining two features in terms of information leakage.


% feature optimization (fast feature selection?)

% I am wondering whether it is possible to construct a specific classifier for a given defense. I am thinking, after the defense, some highly impacted features may do negatively on the classifier performance. But for a attacker, he has the possibility to know which defense is applied and optimize the feature selection. (it's worth noting that most of the researchers is not willing to optimize the classifer's performance in attacking the defense. Defense designers do not do so. The attacker papers change classifers, and no attention has been given to feature selections. There is a possible gap that I can have the change.)


% Step 1: the very first step is to extract all the features. This reminds me that my dataset is not well organized, making recreation un-repeatable. I need to re-organize it to facilitate future twicks.

% I write motivation in the following (making me think clearly)


% the core is ALL
The first contribution is that we measured the information leakage for all the proposed features in website fingerprinting attack literature. As far as we know, this is the first complete information-theoretic measurement over all known features.

Knowing the information leakage of each feature, one can know how much the attacker can narrow down the possibilities.

The second contribution is that we compute the mutual information between a pair of features. We investigate the chemistry between two features. Our finding is that the information leakage for combined features are far complexed. Sometimes the combined features have more information than their summaion; sometimes the combined features have less than the smaller of them. For example, the standard deviation of packet ordering is less than the direct combination of all features.
We investigate the reason why the chemistry may differ. Our finding is that.. This finding gives us guide in constructing the feature set to launch website fingerprinting attacks at the existence of defense.



% feature selection:
% look at random forest and study why k-anonymity outperforms other classifiers in defense case. There might be a clue. 
The third contribution is that our measurement can help in selecting the features in constructing more powerful attackers. When conditions are different, such as at the existence of different kinds of defenses, different prior probabilities, different tor brower version number, bandwidth, different feature set may generate different performance. Our information measurement can give a user a quick way to inspect the features and the features' relations to make up the feaure set for best performance.


 


==> assumption.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.4\textwidth]{graph/multitab.eps}
\vspace{-10pt}
  \caption{\footnotesize Information Leakage with multi-tab
    experiment. The entropy $H(C) = 6.6439$, and the total information
    leakage is $6.6209$. For reference, in the closed-world
    evaluation, The leakage by category were 5.00, 5.34, 6.20, and 3.68}
  \label{fig:multitab}
\vspace{-10pt}
\end{figure}

\section{Exploring Assumptions}\label{sec:assume}
Recently, Juarez {\em et al.}~\cite{critical} enumerated several assumptions
present in WF attack papers, and evaluated the classifiers from
several of these papers under conditions that violate these
assumptions.  Unsurprisingly, the success rates of the classifiers was
greatly reduced, however, as noted in the Introduction, this does not
clearly indicate the degree to which violating these assumptions
reduces the information present in various features.

As an example application of our methodology, we repeated the
multi-tab browsing experiment reported by Juarex {\em et al.}.  For
each Alexa Top 100 page $C$, we loaded $C$ in the foreground, while
randomly choosing another page from the same set to load in the
background at a randomly chosen delay between 0.5 and 5 seconds.  We
collected 100 fingerprints for each page (in 8 batches) and measured
the information present in these fingerprints.

The results (assuming uniform priors) appear in
Figure~\ref{fig:multitab}. Overall, the fingerprint leaks nearly the
same amount of information, but the individual features and categories
change, with directional trigrams leaking slightly more information
and the first 20 packets leaking much less information. It will be
interesting to further evaluate other ecological variables identified
by Juarez {\em et al}, such as TBB versions, TBB settings, and network
variability.


==> bandwidth.tex <==
\section{Bandwidth Selection}


We use the Rule of Thumb to determine the bandwidth of the kernel density estimation when considering a continuous feature variable; when it comes to a discrete feature $f$, we use a very small bandwidth (0.001) to approximate its generic probability density function.

But for a specific webpage, its traffic is characterized to be multi-modal, thanks to varying network conditions, random advertisement or contents, and unpredictable order of resources\cite{usenix_wang}. A feature variable of the webpage consequently may show multiple modes. Such a phenomenon makes kernel denstity estimation oversmooth. In addition, even a feature variable can be discrete in some modes, and continuous in other modes. We find such a phenomenon in traffic defended by BuFLO approach. This makes the problem of oversmoothing even worse.

We solve the oversmoothing problem by law of total probability. Suppose a website has $k$ modes, which are $m_1, m_2, \cdots, m_k$. Then the overall probability density function for a feature variable $\bar{f}$ is 
\begin{equation}
p(\bar{f}|c_j) = \sum_{i = 1}^{k}{ p(\bar{f} |c_j, m_i)p(m_i) }
\end{equation}   
Then we do kernel density estimation on each mode separately. 

\begin{equation}
\begin{split}
\hat{p}_(\bar{f}|c_j) &= \sum_{j = 1}^{k}{\{ \frac{p(m_i)}{|m_j|*h_j} \sum_{p_c \in m_j}K(\frac{\bar{f}-p_c}{h_j}) \} } \\ 
&= \sum_{j = 1}^{k}{\{ \frac{1}{n*h_j} \sum_{p_c \in m_j}K(\frac{\bar{f}-p_c}{h_j}) \} }
\end{split}
\end{equation}

Based on the above observations, we first run clustering algorithm to separate the modes of a webpage, then calculate the bandwidth within each mode, and assign the obtained bandwidth to the kernels of the corresponding mode. 


==> closedworld.tex <==
\section{Closed-world evaluation}\label{sec:closed}

\begin{table}[h!]
\center 
\input{feature-tab}
\vspace{-5pt}
\caption{\footnotesize The information leakage in closed-world with equal priors. The total leaked information $I(F;C)$ is $6.5918$, and the entropy $H(C)$ with equal priors is $6.6294$.}
\vspace{-15pt}
\end{table}
\subsection{Individual features}

The closed-world dataset consists of index pages from the Alexa 100 most visited websites. Each website has 600 traffic instances; the dataset ends up with 60000 traffic instances. We use the Tor-Browser-Crawler~\cite{tor-browser-crawler} to crawl the 100 websites, and extract the cell traces by the method in~\cite{ndss16}. %In order to shorten the crawling time, we start four virtual machines on a host, which individually walk through the Alexa list by visiting a website 30 times. Such crawling is repeated 5 times to collect a website's 600 instance. 



\emph{\textbf{Observation 1:} From packet number, upload stream leaks at least same amount of information ($9.1\%$ more in Shannon entropy) than download stream.}

Web-browsing is characterized by asymmetric traffic. The incoming packets, which contain the requested contents, outnumber the outgoing packets carrying requests. A natural question is does their packet number leak different amount of information as well? Our measurement shows that the upload stream, though having many fewer packets, leaks at least as much of information from packet count as the download stream. The defense design should give same amount of attention to upload stream in hiding both streams' packet number. 

\begin{figure}[t]
  \centering 
  \includegraphics[width=0.45\textwidth]{graph/pktnum_vs_mi_income.eps}
  \includegraphics[width=0.46\textwidth]{graph/pktnum_vs_mi_outgo.eps}
\vspace{-10pt}
  \caption{\footnotesize Packet Count vs. Mutual Information}
  \label{fig:pkt_mi}
\vspace{-10pt}
\end{figure}

\emph{\textbf{Observation 2:} The relationship between packet count and its information leakage is U-shaped.}

We use our closed-world dataset to plot Figure \ref{fig:pkt_mi}. $x$ is the stream's mean packet count in visiting a website, and $y$ is the information leakage from the packet number. We discover that a website generating less than $2000$ or more than $4000$ incoming packets would leak $56.8\%$ or $18.5\%$ more information (in Shannon Entropy) about itself by packet count, and that a user generating less than $200$ or more than $400$ outgoing packets would leak $31.3\%$ or $13.8\%$ more information about the visited website. 

\begin{figure}[t]
  \centering
  \includegraphics[width=0.3\textwidth]{graph/variation_vs_pktnum.eps}
\vspace{-10pt}
  \caption{\footnotesize Packet Count vs. Variation}
  \label{fig:pkt_variation}
\vspace{-10pt}
\end{figure}

We discover two contributors to this phenomenon. The first contributor is the positive correlation between the packet count and its variation, which is shown in Figure \ref{fig:pkt_variation}.  Websites generating more packets tend to see a larger variation in the number of generated packets. The same phenomenon also applies to outgoing packets. As a smaller variation makes the packet count more predictable, streams having fewer packets leak more information from the packet count.  The second contributor is that a website stands out if its packet count is larger than average. This contributor results in the rise of information leakage with the incoming packet volume larger than $4000$ or outgoing packet volume larger than $400$.


\emph{\textbf{Observation 3:} the 3rd burst leaks the most information among the first $5$ bursts.} 

We observe that the 3rd bursts leaks $1.0186$ bit information, much more than the 1st burst ($0.2747$), the 2nd burst ($0.3708$), the 4th burst ($0.6196$), and the 5th burst ($0.7314$).

%% first 20 packet (individual measure) uses bootstrap
%% others use subsampling

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.4\textwidth]{graph/ent2prob_closed.eps}
% \vspace{-10pt}
%   \caption{\footnotesize Anonymity Set Size vs. Entropy: an Equivalent Illustration}
% \vspace{-10pt}
%   \label{fig:ent2prob_closed}
% \end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.3\textwidth]{graph/closed_prior_measure.eps}
\vspace{-10pt}
  \caption{\footnotesize Closed-World: the Measurement with Popularity Related Priors. The total information leakage $I(F;C)$ is $5.2599$, the entropy $H(C)$ with priors is $5.2772$.}
  \label{fig:closed_world_prior_measure}
\vspace{-10pt}
\end{figure}

\subsection{Feature Categories}

\emph{\textbf{Observation 4.} Total Packet Count, Incoming Packet Count, $(-1,-1,-1)$ trigram frequency, and maximum burst are highly correlated.}
The Figure \ref{fig:mi_matrix} shows that these features correlates with each other to the extent that their normalized mutual information is close to $1$. The reason is the asymmetric property of the web-browsing traffic. We observe that the incoming packets outnumbers the outgoing packets on average. The incoming packet count therefore dominates the total packet count, and naturally correlates to the ``all-incoming'' $(-1,-1,-1)$ trigram, and the size of the maximum burst of incoming packets.

\emph{\textbf{Observation 5.} The categories of features that leaks information from the most to the least are bursts, packet order, packet number, and the first 20 packets. }

\subsection{Popularity Priors}

Having estimated the conditional PDFs for all features given equal
priors, it is relatively straightforward to evaluate the effect of
different prior distributions on the information leakage due to
website fingerprints.  Figure~\ref{fig:closed_world_prior_measure}
shows the result of measuring with popularity-based priors.  In this
case, the entropy $H(C)$ is decreased (due to some websites being more
probable than others) and the leakage $I(F;C)$ is correspondingly
decreased, although in both cases $H(C|F)$ is very low ($0.03$ vs
$0.02$). 

We obtain the popularity-based priors by Zipf law~\cite{zipf}. Alexa.com provides websites' ranks without number of visits (at least for free users). \cite{zipf} demonstrates that the website's rank $r$ and its number of visits $v$ follow the Zipf law $v = Cr^{-1}$, where $C$ is a constant. Such relation enables us to estimate the number of visits by a website's rank. Consequently we obtain the priors of websites. Note that knowing the constant $C$ is not necesssary for the estimation.



\emph{\textbf{Observation 6.}  In the closed-world setting, equal
  priors and popularity priors preserve the relative ordering between
  feature categories.}


==> cluster.tex <==
\section{Clustering of fingerprint features}
To cluster the fingerprint features, we apply DBSCAN~\cite{} on the distance matrix. DBSCAN is a density-based clustering algorithm. It assigns a feature to a cluster if this feature's distance from any feature of the cluster is smaller than a threshold $\epsilon$, otherwise the feature starts a new cluster in our setting. Such algorithm guarantees that the distance is bigger than $\epsilon$ between any two features belonging to different clusters, which equivalently means the features' normalized mutual information is below $1-\epsilon$. Thus, we can change $\epsilon$ to adjust the degree of independence between clusters.       
\begin{table*}[t]
\centering
\begin{tabular}{l*{16}{c}r}
\hline
Fingerprint&	1 & 2  & 4  & 6 & 7 & 8 & 10 & 12 & 14 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 \\
Cluster &		2 & 24 & 17 & 2 & 2 & 1 & 12 & 10 & 2  & 11 & 11 & 4  & 4  & 4  & 11 & 25 & 19 \\
\hline
Fingerprint& 	27 & 28 & 29 & 30 & 31 & 32 & 33 & 34 & 35 & 36 & 37 & 38 & 39 & 40 & 41 & 42 & 43 \\
Cluster &	 	15 & 7 & 26 & 3 & 20 & 18 & 22 & 9 & 21 & 23 & 5 & 14 & 27 & 13 & 6 & 16 & 8 \\
\hline				
\end{tabular}
\caption{\footnotesize Result of DBSCAN clustering on fingerprint features}\label{tab:dbscan}
\end{table*}
Table~\ref{tab:dbscan} gives the DBSCAN clustering results when $\epsilon$ equals to $0.6$. DBSCAN creates $27$ clusters, and the largest cluster has $4$ fingerprint bits. 


==> defense.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.4\textwidth]{graph/tamaraw.eps}
\vspace{-10pt}
  \caption{\footnotesize Information Leakage under Tamaraw Defense}
  \label{fig:defense_tamaraw}
\vspace{-10pt}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.4\textwidth]{graph/buflo.eps}
\vspace{-10pt}
  \caption{\footnotesize Information Leakage under BuFLO Defense ($\tau=10$)}
  \label{fig:defense_buflo}
\vspace{-10pt}
\end{figure}


\begin{figure}[t]
  \centering
  \includegraphics[width=0.4\textwidth]{graph/buflo_50.eps}
\vspace{-10pt}
  \caption{\footnotesize Information Leakage under BuFLO Defense ($\tau=50$)}
  \label{fig:defense_buflo50}
\vspace{-10pt}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.4\textwidth]{graph/glove_indiv.eps}
\vspace{-10pt}
  \caption{\footnotesize Information Leakage under Glove Defense (Cluster Number is $10$)}
  \label{fig:defense_glove}
\vspace{-10pt}
\end{figure}


\begin{figure}[t]
  \centering
  \includegraphics[width=0.4\textwidth]{graph/tamaraw_entropy_vs_bins.eps}
\vspace{-10pt}
  \caption{\footnotesize Tamaraw: Entropy for each Partition}
  \label{fig:tamaraw_entropy_vs_bins}
\vspace{-10pt}
\end{figure}

\begin{table*}
\centering\small
\begin{tabular}{ | c | c | c | c | c | c | }
  \hline
  defense & Packet Number & Packet Order & Bursts & First 20 Packets & Total  \\
  \hline
  BuFLO ($\tau=10$) & 3.1293 & 4.0309 & 3.1529 & 0.0000 & 4.5658\\
  BuFLO ($\tau=50$) & 2.6616 & 3.3122 & 2.6925 & 0.0000 & 3.7484\\
  Tamaraw ($L=100$) & 2.6925 & 3.1108 & 2.2582 & 0.0000 & 3.2817\\ 
  Glove (Cluster=10) & 3.0425 & 3.0425 & 3.0425 & 3.0425 & 3.0425 \\
  \hline
\end{tabular}
\vspace{-10pt}
\caption{\footnotesize Website Fingerprinting Defenses: the Information Leakage from
  categories of features}\label{tab:defense}
\vspace{-10pt}
\end{table*}

\section{Evaluating WF Defenses}\label{sec:defense}
WF Defenses, such as BuFLO and Tamaraw, try to limit the information
leakage of traffic features, typically by padding these features to
preset or random values. This section studies how effective the
defenses are, and measure how much information is still leaked.
 

\emph{\textbf{Observation 7.} Applying the BuFLO defense make transmission time leak more information.}
% why timing leaks much less information

The inappropriately configured BuFLO defense may benefit a time classifier attacker\cite{buflo}. We discover that even with proper configuration, BuFLO makes some features leak more information. The fdownload time is a good example. Without any defense, this feature leaks $1.1133$ bits information. But applying the BuFLO defense increases its leakage to $2.4449$ (when $\tau = 10s$) or $1.8877$ (when $\tau = 50s$). 

The fixed interval results in this increase. It makes download time highly correlate with packet count (total, incoming, or outgoing). We find that applying BuFLO increases the normalized mutual information between transmission time and total packet number from $0.1636$ to $0.9865$. The download time consequently leaks similar amount of information as packet count.

\emph{\textbf{Observation 8.} BuFLO only reduces information leakage of the total packet number by $13.98\%$ with $\tau = 10s$ or by $25.46\%$ with $\tau = 50s$.}

Within the threshold time $\tau$, BuFLO successfully covers the traffic's features by the fixed packet length and pre-determined time interval. This is demonstrated by our measurement: the features which are extracted from the early stage of the traffic (such as first 20 packets and first 5 bursts) leaks no information. However, BuFLO does not cover the features of the traffic beyond the threshold time $\tau$; such uncovered features carry rich information to the extent that the total information leakage on average is still $4.5658$ bits when $\tau=10$ and $3.7484$ when $\tau=50$.

\emph{\textbf{Observation 9.} Glove quickly leaks all possible information from the first 20 packets; an attacker therefore does not have to look beyond the first 20 packets for quick detection.   
} 

Glove groups websites into clusters; within each cluster, Glove computes a super trace for this cluster's instances to replay in transmission. While this approach is claimed to guarantee security with less cost, it gives the attacker the chance for early detection. Our measurement discovers that observing the first 20 packets enables an attacker to have all available information, even before the traffic reaches its end. 
  
\emph{\textbf{Observation 10.} The outbound and inbound traffic of Tamaraw still leaks about $2$ bits of information separately.}

Tamaraw partially covers the packet number by padding it to the
multiples of a parameter $L$. We observe that the consequent
information leakage is only reduced from $3.1137$ to $1.8807$ for
outgoing traffic, and from $2.8527$ to $2.2568$ for incoming
traffic. In addition, since the padding are applied separately for
incoming and outgoing traffic, the leaked information of the two
features is not dependent. The total information leakage from the
packet count is $2.6925$ shown in Table \ref{tab:defense}.
 

\emph{\textbf{Observation 11.} Glove leaks same amount of information from different categories of features.
}

We observe that Glove leaks same amount of information from packet number, packet order, bursts, and first 20 packets. Replaying super traces is the cause for such phenomenon.  



==> feature-tab.tex <==
\small
\begin{tabular}{cccc}
\hline
Category & & $I(F;C)$ & Group ($92\%$ CI) \\

\hline
\multirow{3}{*}{Counts} & Total & 2.87 & \multirow{3}{*}{5.00 (4.98,5.02)} \\	
&Out & 3.11  \\
&In & 2.85 \\
\hline
Time &  &  & 1.11 (1.09, 1.13) \\
\hline
\multirow{8}{*}{3-Grams} & ($-,-,-$) & 2.82 & \multirow{8}{*}{5.34 (5.33,5.37)} \\
& ($-,-,+$) & 2.40 \\			% 6
& ($-,+,-$) & 1.87 \\
& ($-,+,+$) & 2.19 \\
& ($+,-,-$) & 2.40 \\
& ($+,-,+$) & 0.61 \\			% 10
& ($+,+,-$) & 2.20 \\
& ($+,+,+$) & 1.99 \\

\hline

\multirow{11}{*}{Bursts} &Max& 0.91 & \multirow{11}{*}{6.20 (6.18,6.21)} \\			% 13
&Ave & 1.52 \\
&Num & 3.12 \\
&\#($>5$) & 2.68 \\
&\#($>10$) & 1.70 \\				% 17
&\# ($>15$) & 2.34 \\
&1st & 0.27 \\
&2nd & 0.37 \\				% 20
&3rd & 1.02 \\
&4th & 0.62 \\
&5th & 0.73 \\					% 23

\hline 

\multirow{20}{*}{Packets} &1& 0.33 & \multirow{20}{*}{3.68 (\texttt{3.67, 3.78})}\\		% 24
&2& 0.34  \\
&3& 0.18 \\
&4& 0.43 \\
&5& 0.39 \\
&6& 0.42 \\
&7& 0.34 \\
&8& 0.29 \\
&9& 0.24 \\
&10& 0.18 \\
&11& 0.19 \\
&12& 0.16 \\
&13& 0.12 \\
&14& 0.20 \\
&15& 0.24 \\
&16& 0.27 \\
&17& 0.26 \\
&18& 0.19 \\
&19& 0.19 \\
&20& 0.18 \\
\end{tabular}

==> frank.tex <==
\section{Total Information Measurement}
In previous section, we have shown how to measure the information leakage of individual features. This section discusses how to quantify the information leakage over multiple features or even overall features. 

The challenge of measuring multiple features is the curse of dimensionality. With more and more features included in the measurement, the accuracy of MKDE in modeling these features would degrade quickly. Such property limits how many features can be included in the measurement. Unfortunately, the number of features for Tor traffic can be large. For example, in our case, we have $3043$ features in total, and in\cite{knn} $3000+$ features are used. How to measure the information leakage for the overall features becomes a challenge due to the curse of dimensionality. 

We use following approaches to overcome this challenge. 



\subsection{Pairwise Mutual Information Analysis}
We measure the pairwise mutual information between any two features. Our results show that some pairs of features share most of the information, while some pairs share very little information, or in other words, they are closer to independence. Based on this observations, we provide two approaches to reduce the dimensions in the measurement. 

\subsubsection{Pruning over high MI pairs.} If a pair of features has mutual information larger than a threshold, we randomly eliminate one of these two features from the feature set and keep the other. 

\subsubsection{Grouping by MI}. as is shown in relevent sections. 

\subsection{Pruning based on Feature Ranking}
we rank the features based on the information leakage of each. We select the top $n$ features, and the measure the information leakage over them. We find that with including more and more features, their information leakage reaches a platau. we can show this in the figure. Other researches such as \cite{kfingerprint} also has similar results. The results shows that top 100 features capture most of the information leakage of overall features.



\section{Feature Rank}
% experiment setup
We measure the information leakage for each feature in the closed world scenario, and we suppose the prior probabilities ($P(C_i)$) for each website to be equal. 
 
% statistics about all features


\begin{figure}[t]
  \centering
  \includegraphics[width=0.45\textwidth]{graph/hist_of_leaked_info.eps}
\vspace{-10pt}
  \caption{\footnotesize hist}
  \label{fig:hist_of_leaked_info}
\end{figure}




Figure X shows the histgram of features' leaked information. We find that $80\%$ features leaks less than  bit information.

% describe the feature rank results


% packet number: rounding is no better than doning nothing: even rounding decreases info of ratios from 1.5 to 0.9.
% transmission time: from 25 percentile to 100 percentile, the information leakage increase, but why?


==> implementation.tex <==
\section{implementation}
\begin{figure}[t]
  \centering
  \includegraphics[width=0.35\textwidth]{graph/implementation.eps}
  \caption{the Implementation of the Information Measurement}
  \label{fig:implementation}
\end{figure}

We implement our information leakage framework by MATLAB scripts. the \texttt{Websiter} and the \texttt{EvaluatorMachine} are two core classes. Websiter represents a website, while EvaluatorMachine containing all the websites by a list \texttt{EvaluatorMachine.WebsiteList}. 

The \texttt{Websiter} class has a member variable \texttt{model}, which contains the probabilistic models for the instance website. To control the types of the measurement (single feature measurement, MKDE, or Kononenko's Algorithm), \texttt{Websiter} includes a \texttt{model\_vec} member variable, indicating the group indice of the features. The features having same group indice would be dealt with by M-KDE, while the features having different indice would be considered independent with each other. The \texttt{model\_vec} is obtained by mutual information measurement over features.
The \texttt{EvaluatorMachine} class has a member variable \texttt{Prior}, which gives the prior probabilities for the websites. It also contains a member variable \texttt{IsOpenWorld}, which specifies whether the experiment is open-world or closed-world.
    
    
The member function \texttt{GenerateSamples()} and \texttt{Evaluate()} are used for information evaluation. The samples are firstly drawed from the probabistic models by \texttt{GenerateSamples()}, and these samples are evaluated by \texttt{Evaluate()}. The function \texttt{reModel()} is used for error measurement. We implemented two methods, bootstrapping and subsampling, for the measurement. \texttt{MI()} function is used for mutual information measurement over all features, feeding the \texttt{model\_vec} with the group indice. 



\subsection{Evalute in Parallel}
% why parallel
The entropy-based evaluation could take days to finish. Such time cost would be more if the evaluation adopts a larger dataset or has more subsampling trials. This section introduces our approach of evaluating in parallel.

The evaluation is comprised of the dataset importing, the probabilistic model building, sampling, and the sample evaluation. We discover that our evaluation tool spends most of its time on evaluating the samples. Based on this observation, we coordinate a collection of machines to evaluate the samples in parallel.
Our distributed computation includes following entities:
\begin{itemize}
\item \emph{a central server}: this server takes charge of the centralized computation, such as the dataset importing, model building, and sampling. In addition, this server acts as the coordinator to instruct workers to evaluate the assigned samples.
\item \emph{a collection of workers}: these workers connect to the central server for receiving the probabilistic model and samples to evaluate. After evaluation, the workers return the evaluation results to the central server for recording. 
\end{itemize}   

To harvest multiple cores in a single machine, we adopt the MATLAB's parallel computing toolbox. Such a toolbox enables us to initiate multiple workers in a single machine. 




% how to parallel




==> individual.tex <==
\section{Information in a single feature} \label{sec:individual}
This section introduces how to quantify a single feature's information leakage--the basis for information measurement upon a complete set or a subset of features. 
Suppose we have a single feature $\bar{f}$, the goal is to quantify its mutual information with the variable $C$. The measurement is shown in the following:

\medskip
\noindent \textbf{MEASUREMENT.} an individual feature $\bar{f}$'s information leakage about the visited website $C$ is:  
\begin{equation} \label{eq:single_feature}
\begin{split}
I(C;\bar{f}) &= H(C) - H(C|\bar{f}) \\
H(C)  &= -\sum_{c_i \in C}{\Pr(c_i)\log_2\Pr(c_i)} \\
H(C|\bar{f}) & =  \int_{\Phi} p(x) H(C|x) dx
\end{split}
\end{equation}
where 

$Pr(c_i)$ is the probability that the visted website is $c_i$,

$\Phi$ is the domain for the feature $\bar{f}$, and

$p(x)$ is the probability density function for variable $x$. 

\medskip

Note that we put the conditional entropy in continuous form. It's due to our approach of modeling the feature's probability distribution in Section \ref{sec:abit}.


The prerequisites for this measurement include: (a) estimating the feature $\bar{f}$'s probability density function (Section \ref{sec:abit}), (b) evaluating the definite integral over the domain of the feature $\bar{f}$ (Section \ref{sec:mc}), and (c) compute the entropy of $C$ conditioned on an observed value of the feature $\bar{f}$ (Section \ref{sec:ent}). We give more details in the following sections. 

%\begin{itemize}[noitemsep]
%\item estimate the probability density function of the random variable $\bar{f}$ (Section \ref{sec:abit}) 
%\item calculate $H(C|x)$ when $x$ is a sampled value of the variable $\bar{f}$ (Section \ref{sec:mc}) 
%\item compute the integral over the domain $\Phi$ (Section \ref{sec:ent}) 
%\end{itemize}

\subsection{Probability Density Function Estimation for a Feature}\label{sec:abit}
The first prerequisite for measuring a feature's information leakage is to model its probability distribution. A popular approach is to use histogram. However, as the traffic features exhibits a great range of variety, it's hard to decide on the number of bins and width. This paper adopts Kernel Density Estimate (KDE)~\cite{rosenblatt1956remarks}, which outperforms histogram in smoothness and continuity.

KDE is a non-parametric method to estimate a random variable's the probability density function. It uses kernel functions--a non-negative functoin that integrates to one and has mean zero--to approximate the shape of the distribution. The estimated probability distribution is:
\begin{equation}
\hat{p}_(\bar{f}|c_j) = \frac{1}{nh} \sum_{c=1}^{m}K(\frac{\bar{f}-p_c}{h})\
\end{equation}
where

$h$ is called the bandwidth in KDE,

$K(\cdotp)$ is the kernel function of a Gaussian, and

$p_1,p_2, \cdots, p_m$ are the observations for $\bar{f}$ in visiting $c_j$

\medskip

Choosing a proper bandwidth $h$ is important for KDE to make an accurate estimate. If a feature is continuous, this paper adopts plug-in estimator\cite{bw_survey} for bandwidth selection. In case of failure, we uses the rule-of-thumb approach~\cite{bw_survey} as the alternative. If the feature is discrete, we let the bandwidth be a very small constant (0.001 in this paper). The choice of the small constant has no impact on the measurement, as long as each website uses the same constant as the bandwidth in its KDE.  

Our KDE may model a discrete feature as if it's continuous. The reason is that the domain of the feature $\bar{f}$ could be very large and requires much more samples than we can collect in order to accurately estimate in discrete. Take total packet number of Facebook.com as an example. We observe $238$ different values from our $600$ samples in the range of $576$ and $1865$. If the feature is processed as discrete, the estimated probability for observed values would be inaccurate, and the missed values would be considered impossbile inproperiately. Our solution is to consider such a discrete feature to be continuous, so that the kernels would smooth the probability distribution estimation and assign an approprient probability to the missed values.

Our KDE is able to distinguishe a continuous-like discrete feature. Take the feature of transmission time as an exmaple. This feature is used to be continuous, but when defenses such as Tamaraw are applied, the feature would come as discrete. Our KDE is able to recognize by two approaches. The first approach is about using a threshold $\beta$. If the same traffic instances are observed more than $\beta$ times in our dataset, these instances are distinguished as discrete cases, and our KDE would take their features to be discrete. The second approach is template matching used in BuFLO case. We precompute a pattern of traffic believed to be discrete, and we consider the instances matching the pattern as discrete. In case of BuFLO, the pattern is the resulted traffic instance with transmission time $\tau$. 

Moreover, our KDE can handle a feature which is partly continuous and partly discrete. Such features exist in BuFLO-defensed traffic. These features would be discrete if the genuine traffic can be completed within time $\tau$, otherwise, the features would be continuous.
Based on~\cite{fruhwirth2006finite,mixture}, we compute the bandwidths separately for discrete and continuous feature values; then we apply adaptive kernel~\cite{van2003adaptive} which allows different bandwidths for kernels in KDE.

%A feature can be partly continuous and partly discrete. In BuFLO defense, if the genuine traffic can be finished within the transmission time $\tau$, the traffic would be padded to be the same traffic template. The features extracted from the traffic are discrete, no matter they are previously discrete or continuous.     



%Though features could be discrete, this paper treat a feature to be continuous. The first reason is that the feature space for a discrete feature is usually very large and requires much more samples than we could collect to make an accurate estimation. Take total packet number as an example.   

%This section introduces the probability density function estimate for the feature $\bar{f}$. Firstly it describes how to estimate $p(\bar{f}|C = c_j)$--the PDF of $\bar{f}$ when the website $c_j$ is known to be visited. Secondly, it shows how to derive the generic PDF $p(\bar{f})$ based on the conditional PDFs.    

%The conditional PDF $p(\bar{f}|C=c_j)$ captures the relative likelihood for the feature $\bar{f}$ to be a given value, given that the website $c_j$ is visited. Assuming thatt $\bar{f}$ is a continuous variable (the total download time, for example), we use kernel density estimation (KDE)~\cite{rosenblatt1956remarks} to estimate the conditional PDF $p(\bar{f}|c_j)$.  
%KDE is a non-parametric method to estimate the probability density function of a random variable. It uses kernel functions--a non-negative function that integrates to one and has mean zero--to approximate the shape of the probability density function: 


%$h$ is called the bandwidth in KDE,

%$K(\cdotp)$ is the kernel function of a Gaussian, and

%$p_1,p_2, \cdots, p_m$ are the observations for $\bar{f}$ in visiting $c_j$

%\medskip

%In the case of $\bar{f}$ being a discrete variable, we treat it as continuous and model its PDF by KDE as well. An alternative method is to consider the feature to be discrete and use histograms instead. However, for the sake of smoothness and continuity of KDE and the difficulty of choosing appropriate bin sizes for histograms, we prefer the KDE approach.

%Taking the case in Figure \ref{fig:info_leak} as an example, the feature $\bar{f}$ is the total packet count, and the conditional PDFs to estimate are $p(\bar{f}|\texttt{facebook.com})$ and $p(\bar{f}|\texttt{google.de})$. The results obtained by KDE are shown in Figure \ref{fig:kde}.

%\begin{figure}[t]
  %\centering
  %\includegraphics[width=0.45\textwidth]{graph/kde.eps}
%\vspace{-10pt}
  %\caption{\footnotesize KDE estimate of the conditional PDFs}
  %\label{fig:kde}
%\vspace{-10pt}
%\end{figure}

%To continue, we describe how to derive the generic PDF $p(\bar{f})$ by conditional PDFs. In our closed-world experiment, we estimate the PDFs of the feature $\bar{f}$ conditioned on each website.    
%By applying the law of total probability, the generic probability density function for $\bar{f}$ without assuming any visited website is:
%\begin{equation}
  %\hat{p}(\bar{f})= \sum_{j=1}^{n} {\hat{p}(\bar{f}|c_j) \Pr(c_j)}
%\end{equation}
%where $\hat{p}(\bar{f}|c_j)$ is the PDF of $\bar{f}$ when the visited website is known to be $c_j$.  Given the prior probabilities of websites, the relative likelihood that the feature $\bar{f}$ takes on a specific value can be obtained. Figure \ref{fig:generic} shows the generic PDF $p(\bar{f})$ for our closed-world dataset assuming equal priors. This generic PDF is the basis of our integral evaluation approach, which we introduce in the following section.


%\begin{figure}[t]
  %\centering
  %\includegraphics[width=0.45\textwidth]{graph/generic.eps}
%\vspace{-10pt}
  %\caption{\footnotesize Generic PDF}
  %\label{fig:generic}
%\vspace{-10pt}
%\end{figure}

\subsection{Monte Carlo Integral Evaluation}\label{sec:mc}
The second prerequisite is to evaluate the definite integral over the domain of the feature $\bar{f}$ in Equation \ref{eq:single_feature}. We use the Monte Carlo method~\cite{ghahramani2002bayesian}, which picks random points in the domain and uses these points to numerically approximate the definite integral:
\begin{equation}\label{eq:monte}
H(C|\bar{f}) \simeq \frac{1}{k} \sum_{i = 1}^{k} {H(C|\bar{f}^{(i)})}
\end{equation}

where

$\bar{f}^{(1)}, \bar{f}^{(2)}, \cdots, \bar{f}^{(k)}$ are the random samples, and 

$k$ is the size of the sample.

\medskip

Note that we apply importance sampling~\cite{importance_sampling}, in which random samples are drawn from the distribution having probability density function $p(\bar{f})$. The sampling process is:
\begin{itemize}[noitemsep]
\item Step 1: decide sampling size. To accurately evaluate the integral by Monte Carlo method, sufficent samples are needed. In this paper, the total number of samples is set to be $k = 5000$. For each website $c_j, j\in \{1, \cdots, n\}$, the number of samples is $k \cdot \Pr(c_j)$.
\item Step 2: Sampling. For each website $c_j$, draw $k \cdot \Pr(c_j)$ samples from its distribution with conditional PDF $p(\bar{f}|c_j)$.
\end{itemize} 

We choose importance sampling over uniform  domain sampling (which would require a different estimation than Equation~\ref{eq:monte}),  since it includes more samples for feature values that are more likely to happen. The benefit is that the ``important'' values in the integration are emphasized for higher precision.

The last missing piece to complete the evaluation in Equation \ref{eq:monte} is, how to calculate the conditional entropy $H(C|\bar{f}^{(i)})$. We introduce the details in the next section.  

\subsection{Entropy of Possible Websites} \label{sec:ent}
This section describes how we calculate $H(C|\bar{f}^{(i)})$, the entropy of $C$ conditioned on a feature sample $\bar{f}^{(i)}$. We've already known that the sample $\bar{f}^{(i)}$ leaks information about $C$, so that the probability of a website being visited would change as well. Obtaining posterior probabilities $\Pr(c_w|f^{(i)})$ is the basis of evaluating the conditional entropy. Based on Bayes' Theorem, we have the posterior probability $\Pr(c_w|f^{(i)})$ for the website $c_w$ being visited:
\begin{equation} \label{eq:bayes}
  \Pr(c_w|\bar{f}^{(i)}) = \frac{\hat{p}(\bar{f}^{(i)}|c_w) \Pr(c_w)}{\sum_{j=1}^{n}{\hat{p}(\bar{f}^{(i)}|c_j)\Pr(c_j)}}
\end{equation}
Note that we adopt the method in~\cite{bouckaert2004naive} to handle a continuous variable in Bayes' theorem; the conditional PDFs $\hat{p}(\cdot)$ are consequently used in Equation \ref{eq:bayes} without converting them to probabilities.

We calculate the posterior probabilities for each website being visited, and we obtain the entropy of possible websites after learning the feature $\bar{f}^{(i)}$:
\begin{equation}
H(C|f^{(i)}) = - \sum_{c_j \in C} \Pr(c_j|f^{(i)}) \log \Pr(c_j|f^{(i)})
\end{equation}
As a result, we can continue to evaluate a feature's information leakage by Equation \ref{eq:monte}.



\begin{figure*}[t]
  \centering
  \includegraphics[width=1\textwidth]{graph/individual_enlarge.eps}
  \caption{\footnotesize Generic PDF}
  \label{fig:generic}

\end{figure*}




%Let's still take the case of \texttt{google.de} and \texttt{facebook.com} as an example. Suppose the sampling size is $200$, which means we draw $100$ random samples from the $\hat{p}(\bar{f}|\texttt{google.de})$ distribution, and $100$ samples from $\hat{p}(\bar{f}|\texttt{facebook.com})$. Suppose among the $200$ samples, the first sample $\bar{f}^{(1)}$ has total packet count of 1022. By Equation \ref{eq:bayes} we have the probability $\Pr(\texttt{google.de}| \bar{f}^{(1)}) = 73.73\%$ and $\Pr(\texttt{facebook.com} | \bar{f}^{(1)}) = 26.27\%$. The conditional entropy $H(C|\bar{f}^{(1)})$ is $0.8308$. By averaging the entropies of $C$ conditioned on 200 samples, we obtain the information leakage from total packet count $I(\bar{f};C) = 0.9364$, which is near the maximum possible information leakage (in this two-website case) of $1$.


==> intro.tex <==
\section{Introduction}

The Tor anonymity network uses layered encryption and traffic relays
to provide private, uncensored network access to millions of users
per day.  This use of encryption hides the exact contents of messages
sent over Tor, and the use of sequences of three relays prevents any single
relay from knowing the network identity of both the client and the
server.  In combination, these mechanisms provide effective resistance
to basic traffic analysis.


However, because Tor provides low-latency, low-overhead communication, it does
not hide traffic features such as the volume, timing, and direction of
communications in a given connection. Recent works~\cite{wang2014effective,ndss16,kfingerprint} has shown that these
features leak information about which website has been visited to the extent
that a passive adversary that records this information is able to recognize the
website with more than $90\%$ accuracy in a closed world of $100$ possible
websites, for example.  Such an attack is often referred to as a Website
Fingerprinting (WF) attack.

In response, several works have proposed defenses that attempt to hide this
information, by padding connections with extra traffic or rearranging the
sequence in which files are requested.  These papers train classifiers based on
altered traffic characteristics, and evaluate the effect of the defense based on
the classification accuracy: if the accuracy of the classifier is reduced, the
defense is validated.


Accuracy equals any misclassification to the failure of the attacker or no information leakage, but chances are that the attacker may determine the correct label after several failed trials, or in other words, information leakage may still exist, though not to the extent that it helps the attacker to narrow down the possibilities to only one. 




More recent studies~\cite{cai2014,kfingerprint} have noted that different features can carry different amounts of information, and designed comparative methods to find the most informative features. These methods have been used to suggest defense techniques based on the most informative features.  However, these methodologies do not give a straightforward way to quantify the relationships between features; for example, feature A might be more informative than features B or C alone, but features B and C together might be more informative than A.




We argue that these coarse-grained evaluations of features and defenses are overly simplistic.  The analysis of new WF attack features and defenses should start with the
question: how much information is leaked? In this paper, we develop WeFDE (for \textbf{We}bsite \textbf{F}ingerprint \textbf{D}ensity \textbf{E}stimation), a methodology for modeling the likelihood functions of website fingerprints, and a set of tools for measuring the information leaked by these fingerprints. We show that low information leakage implies low classification accuracy, but the converse is not necessarily true: in a closed-world setting with $n$ websites, a feature set that yields a classifier with accuracy $\alpha$ could leak information with the uncertain range $(1-\alpha)\log_2 (n-1)$. Further, we give examples of features that have enough combined information leakage to uniquely identify websites under popular defense mechanisms, leading to divergent evaluations of these defense mechanisms.

These observations are based on our application of WeFDE to a comprehensive list of $3043$ features (including, to the best of our knowledge, all features described in the Tor WF literature~\cite{shi2009fingerprinting,kfingerprint,wpes11-panchenko,buflo,ndss16,wang_wpes,cai1,wang2014effective}) extracted from a $211219$ Tor web browsing visits for about $2200$ websites. We quantify the information leakage in various scenarios, from closed-world setting with $100$, $500$, $1000$, or $2000$ websites, to open-world setting with $500$, $1000$, and $2000$ non-monitored websites.  We apply several defense mechanisms to these traces, and use WeFDE to compare the accuracy, overhead and information leakage of these defenses.

The design of WeFDE involves two primary challenges.  The first is the choice of model for the likelihood functions of fingerprint features, which can have a wide range of shapes.
We address this challenge by using adaptive kernel density estimation~\cite{van2003adaptive} to model the probability density function of a feature or a category of features. By allowing kernels to determine their bandwidth separately, we can adaptively model both continuous and discrete density functions.

The second challenge is the ``curse of dimensionality,'' in which the data required to estimate a $d$-dimensional density function scales exponentially in $d$. We address this by introducing a set of dimension reduction approaches. Firstly, given a set of features to model, we measure their pairwise mutual information. After recognizing pairs of highly dependent features, we can exclude some of the features. Secondly, we use Kononenko's Algorithm~\cite{cheng1999comparing,Kononenko} and DBSCAN~\cite{ester1996density} to separate features into sub-groups, which have pairwise mutual information higher than a threshold $\epsilon$ within each group, and lower than this threshold among different groups. Then we apply adaptive kernels for each sub-group with reduced dimensionality. Finally, our experiment shows that including enough highly informative features in the measurement is able to approximate the overall information leakage. This enables us to further reduce the dimensionality of our measurement.

To summarize, the contributions of this paper include:
\begin{itemize}

  \item We introduce WeFDE, a method of estimating the likelihood function of a website fingerprint.  The resulting density functions can be used to measure information present in a fingerprint for a given set of websites, but could potentially be further used in a variety of attacks. For example, it could be combined with prior information about likely destinations to draw Bayesian inferences; or used to inform statistical disclosure-style attacks.

  \item We use WeFDE to perform the first comprehensive information leakage measurement for all $3043$ features proposed in the Tor website fingerprinting literature, based on a large dataset having $211219$ Tor web browsing visits to about $2200$ websites.  We draw conclusions on the relationships between these features, and their implications for WF defense mechanisms.

  \item We apply WeFDE to several recently proposed WF defense mechanisms, to show
  that validating a defense by classification accuracy is flawed. These results demonstrate that accuracy and ranking-based measures of information are unreliable guides to the utility of a defense or comparison between two defenses' security.
\end{itemize}


%The paper is organized as follows: Section~\ref{sec:bg} gives
%background and related work on WF attacks, as well as describing the
%features we investigate in this paper.  Section~\ref{sec:method}
%introduces the high-level details of our methodology, while
%sections~\ref{sec:individual} and~\ref{sec:joint} develop the
%methodology in more detail (details about computing confidence
%intervals and our implementation appear in the Appendix).
%Sections~\ref{sec:closed} and~\ref{sec:open} explore information in
%the basic settings, while Sections~\ref{sec:defense}
%and~\ref{sec:assume} explore the effect of WF defenses and tabbed
%browsing. Finally, we conclude in Section~\ref{sec:conclusion}.


==> joint.tex <==
\section{Joint Information Measurement}\label{sec:joint}
% transition: why joint
The previous section measures the information of a single WF feature. In
this section we describe approaches to measuring the information of joint features. Applying these approaches
can provide information on multi-dimensional features, which may be
represented by several components, and even the whole fingerprint.
Comparing with~\cite{cai2014}, which only measures which feature
conveys more information, our approach reveals exactly how much
information a (group of) feature(s) carries.

When measuring the joint features' information, the difference from a single feature measurement is how to estimate the conditional PDF for the features given that a specific website is visited. Suppose the joint features are represented by $\vec{\mathbf{f}} = (f_1,f_2,\cdots,f_d)$, then the conditional PDF to measure is $p(\vec{\mathbf{f}}|c_j), j\in \{1,\cdots,n\}$.


% sub: joint probability density function
\subsection{Multi-variate Kernel Density Estimation}
The first approach to modeling the probability of the joint features for a specific website, is multi-variate kernel density estimation (M-KDE). Comparing with KDE introduced in Section \ref{sec:abit}, M-KDE still uses a set of kernel functions for approximation, but the function to be estimated has multiple random variables as inputs.          

We describe the M-KDE approach in detail. To begin with, for each instance of a specific website, an corresponding observation about the set of Fingerprint features can be obtained. Let $\vec{\mathbf{p}}_\cdot$ denote this observation. Suppose the specific website has $m$ instances; We have $m$ observations denoted by $\vec{\mathbf{p}}_1, \vec{\mathbf{p}}_2,\cdots,\vec{\mathbf{p}}_m$. Based on these observations, M-KDE approximates the joint conditional probability by:
\begin{equation*}\label{multi_kde}
\hat{p}(\vec{\mathbf{f}}|c_j) = \frac{1}{m} \sum_{i=1}^{m}
{K_H(\vec{\mathbf{f}}-\vec{\mathbf{p}}_i)}\  , \text{where}
\end{equation*}

$K_H(\vec{\mathbf{f}}) = |H|^{-1/2}K(H^{-1/2}-\vec{\mathbf{f}})$

$K(\cdot)$ is a multivariate kernel function, and 

H is a symmetric positive definite matrix known as the bandwidth matrix.

The M-KDE approach is not always applicable. When applying M-KDE to
estimate a high dimensional PDF, we find M-KDE inaccurate. The cause
is the curse of dimensionality: as the dimension of the PDF increases,
M-KDE requires exponentially more observations for accurate estimates;
thus M-KDE is confined to low dimensional PDF estimation.   
%% high dimension: naive bayes
%\subsection{Naive Bayes Method}
%To estimate high dimensional PDFs, we use naive bayes method. Naive
%bayes method assumes that the set of features to measure are
%conditionally independent; the features' probability under the
%condition of a specific website is
%\begin{equation*}
%p(\vec{\mathbf{f}}|c_j) = p(f_1|c_j)p(f_2|c_j)\cdots p(f_d|c_j),
%\end{equation*} 
%By estimating each feature's conditional PDF, we obtain a joint PDF for the set of features.

%The advantage of naive bayes method is twofold. To begin with, it
%requires many fewer observations to achieve an accurate estimate. We
%only estimate a single feature's PDF at a time and thus only apply
%one-dimensional KDE, and avoid approximating the joint PDF. This
%property enables naive bayes to estimate high-dimensional PDFs. Second,
%naive bayes method might be useful even when the assumption of
%conditional independence does not hold, as demonstrated by the success
%of naive bayes classifiers. Naive bayes classifiers face the same
%challenge in estimating the conditionally dependent features'
%probability. However, its high accuracy suggests that naive bayes will
%often give reasonable estimates for the probability. Because of these
%benefits, we adopt naive bayes as our first approach to estimate
%high-dimensional PDFs.  

\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{graph/mi_matrix.eps}
  \caption{\footnotesize Mutual information matrix for the top 100 most informative features}
  \label{fig:mi_matrix}
\end{figure}

% high dimention: grouping by dependency
\subsection{Grouping By Dependency}
A workaround from curse of dimensionality in higher dimension is to adopt naive bayes method, which assumes the set of features to be measured is conditionally independent. Naive Bayes requires many fewer observations, thanks to the features' probability distribution separately estimated. However, in our experiment we find dependence between some features of the website fingerprinting, violating the assumption of Naive Bayes. 

We adopt Kononenko's algorithm (KA)~\cite{cheng1999comparing}, which clusters the highly-dependent features into disjoint
groups. In each group, we model the joint PDF of its features by applying the M-KDE approach. Among different groups, conditional independence is assumed.

Before introducing how to cluster features of the fingerprint into
groups, we first describe our approach to measure the dependence between these
features. We adopt mutual information as the quantifying method, which
gives $0$ if two features are independent, and otherwise a positive
value indicating the degree of dependence. We measure the mutual
information between each pair of features. Figure \ref{fig:mi_matrix} represents the mutual information matrix $M$. Note that each entry $M(c,r)$ in the figure has been normalized by Kvalseth's method~\cite{kvalseth1987entropy}. The normalization is:
\begin{equation*}
M(c,r) = \frac{\mathtt{MI}(c,r)}{max\{\mathtt{MI}(c,c),
  \mathtt{MI}(r,r)\}}\ , \text{where}
\end{equation*}         

$\mathtt{MI}(\cdot, \cdot)$ is the function of mutual information, and

$\mathtt{MI}(c,c)$ is the mutual information of $c$ with itself. 
         
\medskip
 
Since $\mathtt{MI}(r,c)$ is less than or equal to $\mathtt{MI}(c,c)$
and $\mathtt{MI}(r,r)$, $M(c,r)$ is in the range of $[0,1]$. A higher
value of $M(r,c)$ indicates higher dependence between features $r$ and
$c$.


We partition the features into disjoint clusters by dependence. To start with, we
convert the mutual information matrix $M$ into a distance matrix $D$
by $D = \mathbf{1} - M$, where $1$ is a matrix of ones. Consequently,
a feature would have $0$ distance with itself, and its distance to another
feature decreases as their mutual information increases. We apply DBSCAN~\cite{ester1996density} on the distance matrix. DBSCAN is a density-based clustering algorithm. It assigns a feature to a cluster if this feature's distance from any feature of the cluster is smaller than a threshold $\epsilon$, otherwise the feature starts a new cluster in our setting. Such algorithm guarantees that the distance is bigger than $\epsilon$ between any two features belonging to different clusters, which equivalently means the features' normalized mutual information is below $1-\epsilon$. Thus, we can change $\epsilon$ to adjust the degree of independence between clusters.



We model the PDF of the fingerprint by assuming independence between clusters.
Suppose KA partitions the fingerprint $\vec{\mathbf{f}}$ into $k$ clusters, $\vec{\mathbf{g}}_1, \vec{\mathbf{g}}_2, \cdots, \vec{\mathbf{g}}_k$, with each feature belonging to one and only one cluster. To calculate the probability $p(\vec{\mathbf{f}}|c_j)$, we have:
\begin{equation*}
p(\vec{\mathbf{f}}|c_j) = \hat{p}(\vec{\mathbf{g}}_1|c_j) \hat{p}(\vec{\mathbf{g}}_2|c_j) \cdots \hat{p}(\vec{\mathbf{g}}_k|c_j)
\end{equation*}  
where $\hat{p}(\cdot)$ is the PDF estimated by M-KDE or KDE.  

As a hybrid of the M-KDE and Naive Bayes, Kononenko's algorithm avoids
the disadvantages of each. First, Kononenko's algorithm does not have
the incorrect assumption that the fingerprint features are independent. It
only assumes independence between groups, since any two of them have
mutual information below $\epsilon$. Second, Kononenko's algorithm
avoids the curse of dimensionality. The groups in Kononenko's
algorithm have much less features than the total number of features.

\subsection{Dimension Reduction}
Besides the KA method to reduce dimension of the features modeled by M-KDE, we employ two other aporoaches to further reduce the dimension.

The first approach is to exclude features that can be represented by other features. We again use the pairwise mutual information to find pairs of features that have higher mutual information than a threshold ($0.9$ in this paper). Then we prune the feature set by getting rid of one of the features and keeping the other.  

Our second approach is to pick out a number of the most informative features to approximate all features' information leakage. Given a set of features to measure, we sort the features by its individual information leakage. Instead of measuring all features' information leakage, we pick out top $n$ features that leak the most information about the visited websites. The measurement results by varying $n$ are shown in Figure \ref{}. It shows that with $n$ increasing, the top $n$ features' information leakage would increase at first but finally reach a platau. This phenomenon shows that the information leakage of sufficient top informative features is able to approximate that of the overall features. Such observation is also backed by~\cite{kfingerprint}, which discovered that including more top informative features beyond $100$ has little gain for classification. 



\begin{figure*}[t]
  \centering
  \includegraphics[width=1\textwidth]{graph/closed_category.eps}
  \caption{\footnotesize Open-world Experiment:}
  \label{fig:closed_category}
\end{figure*}



==> limitation.tex <==
\section{Limitation}
\subsection{the generality of dataset}
\subsection{Depend on Feature Set}


==> measure.tex <==
\section{Website Fingerprints: how much information is leaked}

% website fingerprints, a intro
The fingerprints of the network traffic refer to the non-content traffic properties, such as the packet length, the time interval of two consecutive packets, and the ordering. Though the content of traffic is hidden from an attacker by usage of secure encryption algorithms, the fingerprints of the traffic can still leak information about which websites a user is browsing. A website fingerprinting attacker can harvest such information to de-anonymize a web browsing user. The exsiting research on the website fingerprinting attack focus on the approach and soundness of such an attack, with proposed defenses to cover the fingerprints. Nevertheless, no work answer this fundamental question: how much information is leaked from the fingerprints of the traffic. 

% the motivation: why it is not sufficient
The importance of this question is shown in the following. 

\noindent{\bf Accurately measure the soundness of the attack.} False positive and negative is used in exsting works to measure the soundness of such attacks. Unfortunately, this metric is far from being accurate. 

\noindent{\bf Measure the effectiveness of WFA defenses.}
\noindent{\bf Measure the impact of the unexpected factors.}

% the challenges (if any)

% our methodology
In this paper, we propose the information theoretic framework to measure how much information is leaked in the website fingerprints. 
% side benefits


==> method.tex <==
% independent from a specific classifier. Look at the information leakage directly.
\begin{figure}[t]
  \centering
  \includegraphics[width=0.4\textwidth]{graph/time.eps}
  \includegraphics[width=0.41\textwidth]{graph/pnum.eps}
\vspace{-5pt}
  \caption{Different features may carry different amount of information: time vs. total packet count}
  \label{fig:info_leak}
\vspace{-10pt}
\end{figure}

\section{Methodology}\label{sec:method}

{\bf Information Leakage.} The features leak information about which website is visited. Total packet count is a good example. Figure \ref{fig:info_leak} shows that visiting \texttt{www.google.de} creates 700 to 1000 packets, while browsing \texttt{www.facebook.com} results in 1100 to 1600 packets. Suppose an attacker passively monitors a Tor user's traffic, and it knows that the user has visited one of these two websites (closed-world assumption). By inspecting the total packet count of the traffic (in the range of 700 to 1000, or 1100 to 1600), the attacker can tell which website is visited. 

Different features may carry different amounts of information. Figure \ref{fig:info_leak} displays the download time in visiting \texttt{www.google.de} and \texttt{www.facebook.com}. The former loads in about 3 to 20 seconds, and the latter takes 5 to 20 seconds; Their distributions of download time are not easily separable. As a result, the attacker learns much less information from the download time than from total packet count in the same closed-world scenario.

This raises question of how to quantify the information leakage for different features. We adopt mutual information\cite{info_book}, which evaluates the amount of information about a random variable obtained through another variable, for this measurement, defined as:

\medskip

\textbf{DEFINITION.} The amount of information that an attacker can learn from the fingerprint of the traffic instance is $I(F;W)$:
\begin{equation}
I(F;W) = H(W) - H(W|F)
\end{equation}

where 

$F$ is a random variable denoting the traffic's fingerprint

$W$ is a random variable about website information

$I(F;W)$ is the mutual information between $F$ and $W$

$H(W)$ is the Shannon entropy of the variable $W$, and

$H(W|F)$ is the conditional entropy of $W$ given $F$.


\medskip
Considering the entropy $H(W)$ is solely determined by the priors of each website being visited, the key of the measurement is to determine the conditional entropy $H(W|F)$. The following sections describe how to measure $H(W|F)$ when $F$ is a single feature or a set of features, respectively.




==> new_intro.tex <==
\section{Introduction}

The Tor anonymity network uses layered encryption and traffic relays
to provide private, uncensored network access to millions of users
per day.  This use of encryption hides the exact contents of messages
sent over Tor, and the use of sequences of three relays prevents any single
relay from knowing the network identity of both the client and the
server.  In combination, these mechanisms provide effective resistance
to basic traffic analysis.


However, because Tor provides low-latency, low-overhead communication, it does
not hide traffic features such as the volume, timing, and direction of
communications. Recent works~\cite{wang2014effective,ndss16,kfingerprint} have shown that these
features leak information about which website has been visited to the extent
that a passive adversary that records this information is able to train a classifier to recognize the
website with more than $90\%$ accuracy in a closed-world scenario with $100$ websites. This attack is often referred to as a Website
Fingerprinting (WF) attack. 
In response, many works~\cite{wang2014effective,buflo,cai2014,glove,decoypage,morphing,pipelining,wpes14-csbuflo,cherubin2017website,wang2015walkie} have proposed defenses that attempt to hide this
information, by padding connections with extra traffic or rearranging the
sequence in which files are requested. 

\medskip







\noindent \textbf{Defense Evaluation.} To evaluate a defense, the popular practice is to train classifiers based on altered traffic characteristics and evaluate the effect of the defense by classification accuracy. If the accuracy of the classifier is low enough, the defense is believed to be secure; one defense is believed to be better than another if it results in lower accuracy. 

We argue that \emph{validating defense by accuracy is flawed}. Accuracy is all-or-nothing: classifiers output a single guess and if it is wrong, this is judged to mean the defense has been successful. But this judgement relies on the choice of classifier, and also ignores cases where a classifier may confuse some pages with a small set of others. In such situations, an attacker may well be able to significantly reduce the set of likely pages represented by a fingerprint, even if they cannot reliably choose the correct page from among this set.  We can see that the fingerprint can contain a great deal of {\em information} about the web page even if the classifier cannot accurately identify the correct page.  Thus validating a defense by accuracy is prone to {\em underestimate} its information leakage. 





%\begin{wrapfigure}{R}{0.24\textwidth}
%\end{wrapfigure}
\begin{figure}
\centering
\includegraphics[width=0.36\textwidth]{graph/accuracy/acc_vs_inforange.eps}
\caption{Accuracy vs. Information Leakage: closed-world of 100 websites}\label{fig:acc_vs_inforange}
\end{figure}


We prove that in a closed-world setting with $n$ websites, a feature set yielding a classifier with accuracy $\alpha$ could leak information with the uncertain range $(1-\alpha)\log_2 (n-1)$ (the difference between the maximum and minimum). Figure \ref{fig:acc_vs_inforange} shows when $n=100$ and $\alpha = 0.05$, the possible leakage could be as high as 6.36 bits and as low as 0.06 bits. To conclude, low information leakage implies low classification accuracy, but the converse is not necessarily true: accuracy is not a reliable metric to prove the effectiveness of a defense.

%\begin{figure}[t]
%  \centering
%  \includegraphics[width=0.35\textwidth]{graph/accuracy/acc_vs_inforange.eps}
%  \caption{Accuracy vs. Information Leakage. Suppose a closed-world scenario of 100 websites.}
%  \label{fig:acc_vs_inforange}
%  \vspace{-10pt}
%\end{figure}
   
   

   
   
   
   
   

\medskip

\noindent \textbf{Feature Evaluation.} Different features may carry different amounts of information. WF defense designers can evaluate features to find more informative ones to hide~\cite{cai2014}; attackers can do so to discover highly informative features and optimize their feature set~\cite{kfingerprint}. Existing works~\cite{cai2014,kfingerprint} designed comparative methods to rank the features by their information leakage, but these methodologies do not give a straightforward way to quantify the {\em relationships} between features. How much information do features A and B share? If feature A is more informative than features B or C alone, are features B and C together more informative than A? These methodologies are unable to answer these questions.  


\medskip

\noindent \textbf{Information Leakage Measurement.}
We argue that these coarse-grained evaluations of features and defenses are overly simplistic. The analysis of new WF attack features and defenses should start with the question: how much information is leaked? To answer this question, two challenges should be addressed.  The first challenge is finding a way to model the behavior of WF features and the interaction between them; these features can have highly complex relationships and behavior, exhibiting distributions that could be discrete, continuous, or even partly discrete and partly continuous.  The second challenge is the curse of dimensionality when estimating the total information leakage, as the state-of-art feature sets are usually high-dimensional.  Unfortunately, existing works~\cite{cav,mather2012pinpointing} limited their experimental measurement to features' {\em individual} information leakage, and they cannot overcome these challenges.    

\medskip

\noindent \textbf{Our work.}
In this paper, we develop WeFDE (for \textbf{We}bsite \textbf{F}ingerprint \textbf{D}ensity \textbf{E}stimation), a methodology for modelling the likelihood functions of website fingerprints, and a set of tools for measuring the information leaked by these fingerprints.  The design of WeFDE addresses both of these primary challenges. The first is the choice of model for the likelihood functions of fingerprint features, which can have a wide range of shapes.
We address this challenge by using adaptive kernel density estimation~\cite{van2003adaptive} to model the probability density function of a feature or a category of features. By allowing kernels to determine their bandwidth separately, we can adaptively model both continuous and discrete density functions; by estimating multi-dimensional kernels over sets of features, we can model the interactions between features.

The second challenge is the ``curse of dimensionality,'' in which the data required to estimate a $d$-dimensional density function scales exponentially in $d$. We address this by introducing a set of dimension reduction approaches. Firstly, given a set of features to model, we measure their pairwise mutual information. After recognizing highly dependent features, we exclude the redundant ones. Secondly, we use Kononenko's Algorithm~\cite{cheng1999comparing,Kononenko} and DBSCAN~\cite{ester1996density} to separate features into sub-groups, which have pairwise mutual information higher than a threshold $\epsilon$ within each group, and lower than $\epsilon$ among different groups. Then we apply adaptive kernels for each sub-group with reduced dimensionality. Finally, our experiment shows that by including enough highly informative features in the measurement we are able to approximate the overall information leakage. This enables us to further reduce the dimensionality of our measurement.

We apply WeFDE to a comprehensive list of $3043$ features (including, to the best of our knowledge, all features in the Tor WF literature~\cite{shi2009fingerprinting,kfingerprint,wpes11-panchenko,buflo,ndss16,wang_wpes,cai1,wang2014effective}) extracted from a $211219$ Tor web browsing visits for about $2200$ websites. We quantify the information leakage in various scenarios, from closed-world setting with $100$, $500$, $1000$, or $2000$ websites, to open-world setting with $500$, $1000$, and $2000$ non-monitored websites.  We apply several WF defenses to these traces, and use WeFDE to compare their accuracy and information leakage. Our experimental results demonstrate the unreliability of accuracy in evaluating WF defenses. We also find that the information leakage of WTF-PAD~\cite{juarez2016toward} is unusually high. Interestingly, recent work~\cite{2018arXiv180102265S} confirms our measurement by achieving $90\%$ classification accuracy against WTF-PAD. This demonstrates the advantage of our approach in measuring WF defenses.

\medskip

\noindent \textbf{Contributions}. The contributions of this paper include:
\begin{itemize}
  \item We introduce WeFDE, a method of estimating the likelihood function of a website fingerprint. The resulting density functions can be used to measure information present in fingerprints for a given set of websites, but could potentially be further used in a variety of attacks. For example, it could be combined with prior information about likely destinations to draw Bayesian inferences; or used to inform statistical disclosure-style attacks.

  \item We use WeFDE to perform information leakage measurement for all $3043$ features proposed in the Tor website fingerprinting literature, based on a large dataset having $211219$ Tor web browsing visits to about $2200$ websites. As far as we know, our work is the first large-scale information leakage measurement in the literature. We draw conclusions on the relationships between these features, and their implications for WF defense mechanisms.

  \item We apply WeFDE to several recently proposed Tor WF defense mechanisms, to show
  that validating a defense by classification accuracy is flawed. These results demonstrate that accuracy and ranking-based measures of information are unreliable guides to the utility of a defense or comparison between two defenses' security.
\end{itemize}


The paper is organized as follows: Section~\ref{sec:bg} and Section~\ref{sec:related} give background and related works on WF attacks and defenses, with Section~\ref{sec:features} introducing the
features we investigate in this paper.
Section~\ref{sec:system} introduces the system design of WeFDE.
Section~\ref{sec:closed}, Section~\ref{sec:validation}, Section~\ref{sec:open}, and Section~\ref{sec:info_acc} give information leakage measurement results, and Section~\ref{sec:discuss} provides discussions. Finally, we conclude in Section~\ref{sec:conclusion}.


==> observe.tex <==
\section{Observations}


\emph{\textbf{Observation 1:} From packet number, upload stream leaks at least same amount of information ($9.1\%$ more in Shannon entropy) than download stream.}

Web-browsing is characterized by Asymmetric traffic. The incoming packets, which contain the requested contents, outnumber the outgoing packets carrying requests. A natural question is does their packet number leak different amount of information as well? Our measurement shows that the upload stream, though having much less packets, leaks at least same amount of information from packet number than download stream. The defense design should give same amount of attention to upload stream in hiding both streams' packet number. 


\emph{\textbf{Observation 2:} The relationship between the packet number and its information leakage is U-shaped.}

We use our closed-world dataset to plot Figure \ref{fig:pkt_mi}. $x$ is the stream's mean packet number in visiting a website, and $y$ is the information leakage from the packet number. We discover that a website generating less than $2000$ or more than $4000$ incoming packets would leak $56.8\%$ or $18.5\%$ more information (in Shannon Entropy) about itself by packet number, and that a user generating less than $200$ or more than $400$ outgoing packets would leak $31.3\%$ or $13.8\%$ more information about the visited website. 

We discover two contributors to this phenomenon. The first contributor is the positive correlation between the packet number and its variation, which is shown in Figure \ref{fig:pktnum_variation}. The websites generating more packets tend to see a larger variation in the number of generated packets. The same phenomenon also applies to user-generated outgoing packets. As a small variation makes the packet number less obfuscated, the stream having less packets leaks more information from the packet number.     


%Let's take a website's generated packets (incoming packets) as an example. We observe that websites generating less than $2000$ packets experience $9.37\times 10^4$ variation on average in their packet number. The variation for websites generating more than $2000$ but less than $4000$ packets and websites generating more than $4000$ packets is $3.94\times 10^5$ and $1.19\times 10^7$, respectively. Smaller variation in packet number favors the attacker, leaking more information about the visited websites. 

The second contributor is that a website stands out if its packet number is larger than average. This contributor results in the rise of information leakage with the incoming packet number larger than $4000$ or outgoing packet number larger than $400$. To conclude, such two contributors makes the relationship between the packet number and its information leakage be U-shaped.  




\begin{figure}[t]
  \centering
  \includegraphics[width=0.45\textwidth]{graph/pktnum_vs_mi_income.eps}
  \includegraphics[width=0.46\textwidth]{graph/pktnum_vs_mi_outgo.eps}
  \caption{Packet Number vs. Mutual Information}
  \label{fig:pkt_mi}
\end{figure}




\begin{figure}[t]
  \centering
  \includegraphics[width=0.3\textwidth]{graph/variation_vs_pktnum.eps}
  \caption{Packet Number vs. Variation}
  \label{fig:pkt_variation}
\end{figure}


\emph{\textbf{Observation 3.} Total Packet Number, Incoming Packet Number, $(-1,-1,-1)$ gram, and the maximum burst are highly correlated.}
The Figure \ref{fig:mi_matrix} shows that these features correlates with each other to the extent that their normalized mutual information is close to $1$. The reason is the asymmetric property of the web-browsing traffic. We observe that the incoming packets outnumbers the outgoing packets by XX folds on average. The incoming packet number therefore dominately influences the total packet number, the $(-1,-1,-1)$ gram, and the maximum bursts of the incoming packets.




\emph{\textbf{Observation 4.}	Applying BuFLO and Tamaraw defenses make transmission time leak more information.}
% why timing leaks much less information



\emph{\textbf{Observation 5.} Tamaraw only reduces the information leakage of the packet number by $XX\%$.
% why the packet number are not well protected
}

\emph{\textbf{Observation 6.} }



==> theorem2.tex <==
\section{Proof of Theorem 2} \label{app:theorem2}
Let's denote the information leakage in each closed-world setting to be:
\begin{equation}
  I_l = log_2(n) + \sum_{l\in \{1,\cdots,n\}}{q_l(i)log_2(q_l(i))}
\end{equation}
, where $q_l(i)$ is the probability of visiting the $ith$ website in the $lth$ closed-world setting conditioned on $F = \bar{f}$.

In the combined closed-world setting, the information leakage of $F = \bar{f}$ is
\begin{equation}
  \begin{split}
    & log_2(nx) + \sum_{l\in \{1,\cdots,x\}}{\{\sum_{i\in \{1,\cdots,n\}}{\frac{q_l(i)}{x}log_2(\frac{q_l(i)}{x})}\}} \\
    &= log_2(n) + \frac{1}{x} \sum_{l\in \{1,\cdots,x\}} {\sum_{i\in \{1,\cdots,n\}}{q_l(i)log_2(q_l(i))}}  \\
    &= \frac{I_1 + I_2 + \cdots + I_x}{x}
\end{split}
\end{equation}


==> whyentropy.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.4\textwidth]{graph/possibility_rank.eps}
  \caption{\footnotesize Accuracy-based metrics are not accurate. We adopt the KNN classifier and the closed-world dataset from ~\cite{wang2014effective}. We use $60$ instances of each website for distance learning; we use the other $30$ instances for classification. For a specific test instance, we run the KNN classifier to determine the label in one round; we eliminate the data with this label in next round to determine the next possible label. By repetition, we obtain an ordered list of possible labels. We show where the true label posits in this list.}
  \label{fig:possibility_rank}
\end{figure}

% 1st
% only a draft figure
% possible refinement is to draw cdf, and shade the 1st, 1st-5th, 1st-10th to display how distorted accuracy is. 

% 2nd
% the possibility rank is confusing, find way to explain

% 85.29%    anonymity size of 10
% 76.40%    anonymity size of 5


\section{Accuracy is not accurate}
% how accuracy is used (background)
The accuracy-based metrics are dominant. Not only the website fingerprinting attacks used such metrics to validate their success, but also the defense designs and the critical evaluation tried to prove the failure of WF attacks by the same metrics. However, our experimental result shows that using the accuracy-based metrics to invalidate the WF attacks is flawed. 

Due to its ``all-or-nothing'' nature, the accuracy-based metrics fail to count the ``imperfect'' information leakage of the website fingerprints. 
When the leaked information of a test instance is not ``perfectly'' sufficient, a classifier would fail to pinpoint the exact label of the instance; accuracy-based metrics would therefore count it as a failure (or in other words, as if no information is leaked from the instance). Such distortion results in the under-estimation on the leaked information. 

We conducted an experiment to evaluate the extent of such under-estimation. We focus on the closed-world scenario with a world-size $100$. We use the KNN classifier to analyze the Tamaraw-defended traffic (Tamaraw parameter $L = 100$). The accuracy is $6.87\%$. However, we observe that for $29.1\%$ or $46.67\%$ of the test instances, their information leakage enables the classifier to narrow down the possible websites from $100$ to $5$ or $10$, respectively. When we consider these instances as instances of leaking information, accuracy-based metrics fail to count $76.4\%$ or $85.29\%$ of them. Such under-estimation makes us doubt on the methodology of using accuracy-based metrics to demonstrate the effectiveness of WF defenses or the attackers' failure in the real-world evaluation.


\section{Using Classifiers to validate denfeses are Flawed}
% existing situations 
The defenses against the website fingerprinting attacks are validated by classifiers. Classifiers perform on the defensed traffic, and the defense would be considered effective if the classification accuracy is sufficiently low. 

% problem 
Since the obtained accuracy depends on which classifier is adopted, a problem with such a methodology is that the obtained accurate rate is only a lower bound. A classifier's low accurate rate doesn't guarantee that other classifiers wouldn't perform better. As a result, using the accurate rate of a specific classifier cannot validate the effectiveness of the defense. A recent example is k-anonymity. ~\cite{bufflo} used five classifiers to validate the BuFLO defense: with an overhead of $197.5\%$, the achieved highest accurate rate is $9.4\%$. But \cite{kanonymity} demonstrates that its classifier  

% 




% what's the problem

